Reputation-Driven Adoption and Avoidance of Algorithmic Decision Aids in Credence Goods Markets

In credence goods markets such as health care or repair services, consumers rely on experts with superior information to adequately diagnose and treat them. Experts, however, are constrained in their diagnostic abilities, which hurts market efficiency and consumer welfare. Technological breakthroughs that substitute or complement expert judgments have the potential to alleviate consumer mistreatment. This article studies how competitive experts adopt novel diagnostic technologies when skills are heterogeneously distributed and obfuscated to consumers. We differentiate between novel technologies that increase expert abilities, and algorithmic decision aids that complement expert judgments, but do not affect an expert's personal diagnostic precision. When consumers build up beliefs about an expert's type through repeated interactions, we show that high-ability experts may strategically forego the decision aid in order to escape a pooling equilibrium by differentiating themselves from low-ability experts. Without future visits, signaling concerns cause all experts to randomize their investment choice, leading to under-utilization from low-ability experts and over-utilization from high-ability experts. Results from two online experiments support our hypotheses. High-ability experts are significantly less likely than low-ability experts to invests into an algorithmic decision aid if reputation building is possible. Otherwise, there is no difference, and experts who believe that consumers play a signaling game randomize their investment choice.

==> tab_tex/other-regressions.tex <==
\begin{table}[H]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Even More Regressions}
\begin{tabular}{l*{5}{c}}
\toprule
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
&\multicolumn{1}{c}{\specialcell{First
\\Outcome}}&\multicolumn{1}{c}{\specialcell{Second\\Outcome}}&\multicolumn{1}{c}{\specialcell{Third\ldots}}\\
\midrule

\\
\multicolumn{4}{c}{A. Top Panel} \\
\\
Post &     0.0000\sym{***}&  0.0000\sym{***}&  0.0000\sym{***}  \\
Transition  & (0.0000)         & (0.0000)         & (0.0000)    \\
\\
Mean       &     0.00         &     0.00         &   0.00   \\
$N$          &0,000,000         &0,000,000          &0,000,000   \\
\\
\multicolumn{4}{c}{B. Bottom Panel } \\
\\
Post &     0.0000\sym{***}&  0.0000\sym{***}&  0.0000\sym{***}  \\
Transition  & (0.0000)         & (0.0000)         & (0.0000)    \\
\\
Mean       &     0.00         &     0.00         &   0.00   \\
$N$          &0,000,000         &0,000,000          &0,000,000   \\
\bottomrule
\end{tabular}
\label{tab:regressions}
\vspace*{0.09cm}
\begin{minipage}{0.95\textwidth} 
{\footnotesize 
This table presents\ldots
 \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}
\end{minipage}
\end{table}


==> tab_tex/regressions.tex <==
\begin{table}[H]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Our Regressions}
\begin{tabular}{l*{5}{c}}
\toprule
&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
&\multicolumn{1}{c}{\specialcell{First
\\Outcome}}&\multicolumn{1}{c}{\specialcell{Second\\Outcome}}&\multicolumn{1}{c}{\specialcell{Third\ldots}}\\
\midrule

\\
\multicolumn{4}{c}{A. Top Panel} \\
\\
Post &     0.0000\sym{***}&  0.0000\sym{***}&  0.0000\sym{***}  \\
Transition  & (0.0000)         & (0.0000)         & (0.0000)    \\
\\
Mean       &     0.00         &     0.00         &   0.00   \\
$N$          &0,000,000         &0,000,000          &0,000,000   \\
\\
\multicolumn{4}{c}{B. Bottom Panel } \\
\\
Post &     0.0000\sym{***}&  0.0000\sym{***}&  0.0000\sym{***}  \\
Transition  & (0.0000)         & (0.0000)         & (0.0000)    \\
\\
Mean       &     0.00         &     0.00         &   0.00   \\
$N$          &0,000,000         &0,000,000          &0,000,000   \\
\bottomrule
\end{tabular}
\label{tab:regressions}
\vspace*{0.09cm}
\begin{minipage}{0.95\textwidth} 
{\footnotesize 
This table presents\ldots
 \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}
\end{minipage}
\end{table}


==> tab_tex/summary_stats.tex <==
\begin{table}[H]
    \begin{center}
    \caption{Summary Statistics}
    \begin{tabular}{lcccc} 
    \toprule
    & Group & Group & Group \\
    & 1 & 2 & 3 \\
    \midrule
    Number of people \\
    in the sample & 000,000 & 000,000 & 000,000  \\
    \\
    Mean of the \\
    outcome & 00.00 & 00.00 & 00.00 \\
    \bottomrule
    \end{tabular}
    \label{tab:summary_statistics}
    \end{center}
    
	\begin{minipage}{0.90\textwidth} 
	{\footnotesize 
    This table presents summary statistics \ldots
	\par}
	\end{minipage}
\end{table}

